On-Device CPU Scheduling for Sense-React Systems

Sense-react systems (e.g. robotics and AR/VR) have to take highly responsive real-time actions, driven by complex decisions involving a pipeline of sensing, perception, planning, and reaction tasks. These tasks must be scheduled on resource-constrained devices such that the performance goals and the requirements of the application are met. This is a difficult scheduling problem that requires handling multiple scheduling dimensions, and variations in resource usage and availability. In practice, system designers manually tune parameters for their specific hardware and application, which results in poor generalization and increases the development burden. In this work, we highlight the emerging need for scheduling CPU resources at runtime in sense-react systems. We study three canonical applications (face tracking, robot navigation, and VR) to first understand the key scheduling requirements for such systems. Armed with this understanding, we develop a scheduling framework, Catan, that dynamically schedules compute resources across different components of an app so as to meet the specified application requirements. Through experiments with a prototype implemented on a widely-used robotics framework (ROS) and an open-source AR/VR platform, we show the impact of system scheduling on meeting the performance goals for the three applications, how Catan is able to achieve better application performance than hand-tuned configurations, and how it dynamically adapts to runtime variations.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typset multiple affiliations (Christoph Sommer)

==> old/background-old.tex <==
% applications : illixr, navigation 1para each
% compute limitation etc
% TRY 3-4 PAGES [DAG for all 3 applns]

\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figures/obj_track_dag.png}
\caption{DAG representing the face tracking robot application}
\label{fig:objtrack-dag}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figures/nav2d-dag.png}
\caption{DAG representing the robot navigation application}
\label{fig:nav2d-dag}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.4\textwidth]{figures/illixr-dag.png}
\caption{DAG representing the VR application in iLLIXR}
\label{fig:illixr-dag}
\end{figure}

\subsection{Overview of Robot and XR systems}
\label{sec:appl_overview}
Most robotics and AR/VR applications can be characterized by components connected in a DAG, where each node represents a computation task (or component) and each edge represents flow of data between tasks. Different applications vary greatly in their complexity, based on the high-level task to be accomplished. In this section, we take a look at 3 such applications, and also discuss the task - specific goals for each of them.

\subsubsection{Face Tracking Robot}

A simple face-tracking application~\cite{goebel-2013, ros-face-tracking} is comprised of nodes arranged in linear pipeline (Figure~\ref{fig:objtrack-dag}) -- a camera (C) to capture and pre-process images, a perception node (OD) to find the face in the image, a planning node (VP) to compute the velocity at which the camera must rotate to track the face, and the camera motor that rotates accordingly.

\paragraphb{Performance Goals} The main goal of this robot is to always keep the object in its camera frame, or equivalently, to never lose track of the object.

% In more complex applications, the linear pipeline evolves into a multi-chain DAG.

\subsubsection{Robot 2D Navigation}
The robot's task in this application is to explore an unknown area~\cite{nav2d}. Figure ~\ref{fig:nav2d-dag} represents how the various components within the application are connected to form a DAG.  It uses two sensors -- a laser scanner and an odometer, which reports speed and location information at a high rate to all other nodes. The local cost mapper (LC) uses the laser scans to update its knowledge of the robot's immediate vicinity. The global map and localize node (GML) performs two tasks: (a) Correcting the robot's location and (b) pre-processing the laser scans
% corrects the robot's location obtained from the odometer, and pre-processes the laser scans 
before sending them to the global mapper (GM) that maintains a global map of all the areas that the robot has explored so far. 
The global planner (GP) computes the global trajectory of the robot, i.e. which area to explore next, based on the current position of the robot and GM's global map.
The Navigation Command (NC) node, based on the robot's position and the current trajectory (GP's output), decides in what direction should the robot move.
% which is translated into a direction by the navigation command node (NC). 
Finally, the local planner (LP) uses the local cost map and the navigation command to output the robot's velocity, which is actuated by the mobile base.

\paragraphb{Performance Goals} For the navigation application in a dynamic environment, avoiding obstacles is critical, and that is the first performance goal that we consider. A second goal is to explore the entire area quickly, i.e. to have a high rate of exploration.

\subsubsection{Virtual Reality} The VR application's task is to provide a smooth visualization of the virtual world, based on the user's head movement. Figure ~\ref{fig:illixr-dag} represents the various components within the application. It uses two sensors -- an IMU, which measures acceleration of the user's head, and a camera, which takes pictures of the surrounding environment. The SLAM component fuses the camera and IMU sensors to produce an estimate of the user's pose. The integrator (Int) integrates incoming IMU samples
from the IMU to obtain a relative pose, and combines it with SLAM's output to get a better pose estimate. The Render task (R) uses this pose along with Int outputs to computes an image (aka `frame') of the virtual world, which would be from the perspective of the pose estimate. The Timewarp component takes in this rendered frame and processed IMU values from Int, and updates the frame according to the user's pose based on the IMU data from Int. Lastly, the timewarp's output is sent to the display driver so as to display the frame on a screen mounted to the user's headset.

\paragraphb{Performance Goals}
To provide a smooth virtual visualization, the application should estimate the user's pose correctly [so that the rendered image is in the correct perspective], generating the right image and updating the virtual world state with as less delay as possible. For example, in a bowling simulation, the application should quickly detect if a player crosses the fault line so as to update the scores accordingly.
% player might lose points if they cross the fault line.

% The main goal of the application is to provide a smooth visualization, which requires estimating the user's pose correctly [so that the rendered image is in the right pose], the accuracy of the displayed image w.r.t 

\subsection{Deployment Platforms}
In many low cost robots, sensors and actuators are attached to a single on-board computer which runs all software components in the DAG, often using CPU as the only compute resource~\cite{turtlebot, locobot, turtlebot3}. GPUs and other accelerators can be attached at the cost of higher expense and battery usage. Note that this means that there would be contention among the different components for usage of the CPU. 

In larger robot systems, the nodes may be split across multiple on-board machines~\cite{fetch-doc, earthsense}, or
some nodes may be offloaded to edge or cloud servers~\cite{cloudrobotics, cloudrobotics2, rapyuta, fog-robotics}.

There are some VR headsets which offload the computation to an attached server ~\cite{htcvivepro}.
But more commonly, many AR/VR applications are run with the support of an embedded system ~\cite{qualcommVRPlatform, nvidiajetson, snapdragon835}, on stand-alone devices such as Oculus Go \& Quest ~\cite{oculus-go, oculus-quest}. The embedded platforms provide on-board compute in the form of CPUs, GPUs and accelerators such as DSPs.

In this work, we focus on systems using a single on-board computer, with CPU as the only contended compute resource.

\subsection{Development Frameworks}
It is common to use a software \emph{framework} (e.g.~\cite{orocos, lcm, ros, corba, yarp, nvidia-isaac, HuzaifaDesai2020, openxr}) for developing sense - react applications for both robotics and AR/VR.
The modularity of such frameworks allow developers to easily re-use existing software packages, swapping specific nodes with newer ones, as needed.

Robot Operating System (ROS)~\cite{ros, ros-paper} is by far the most popular framework for robotics applications, with more than 300K estimated users~\cite{ros-metrics}. 
It is widely used for developing research prototypes, with industry usage also growing rapidly~\cite{kiwi, fetch, clearpath, aws-robomaker, ros-cruise}.
% In ROS, each component can be implemented as either a node (i.e. a separate process) or a nodelet (thread within a process).

Illinois Extended Reality testbed (ILLIXR)~\cite{HuzaifaDesai2020} is a new development framework for AR/VR applications, which provides the implementation for various widely used components, along with an extensible communication interface and runtime. It is compliant with OpenXR ~\cite{openxr}, which is a standard for a standard for XR device runtimes to interface with the applications that run on them.
% All components are developed as plugins (or threads) within the same process.

Both the frameworks allow developers to program each component of an application individually, and provide APIs for communication (i.e. flow of data) among those components. 
% There are two broad types of communication supported by both ROS and ILLIXR, listed below. Let us consider there is an edge from component A to B in the DAG of an application [i.e. A's outputs are used by B]. Then, 

% \begin{itemize}
%     \item \paragraphi{Synchronous} B is synchronous w.r.t. A (or equivalently this edge is synchronous) if it waits for A's outputs and executes exactly once for each output of A. This is similar to the publish subscribe or event driven messaging~\cite{seda, rabbitmq} and can be modelled as a message queue b/w A&B with insertions by A and deletions by B. One can set the maximum queue length as a parameter in ROS.
    
%     \item \paragraphi{Asynchronous} B is asynchronous w.r.t. A (or this edge is asynchronous) if it uses the latest output of A every time it executes. 
%     % Illixr's communication interface has support for this, but     % Illixr supports, but ros' commn apis can be used to implement this behavior.
% \end{itemize}

% Note that each component's execution can either be triggered~\footnote{The node executes once for every trigger it receives.} by a synchronous edge or have a periodic timer based on a tunable frequency parameter.

ROS supports using TCP/UDP for communication among different components if they are in different processes, and using shared memory if they are different nodelets within the same process. ILLIXR supports shared memory communication since all components are implemented as different plugins (threads) in the same process.

% TODO: WHERE low level metrics [lat, tput] of these applns?


==> old/design-old.tex <==
\label{sec:design}
\subsection{Problem Formulation}
We model our scheduling problem as meeting constraints on and/or optimizing a weighted linear combination of the low-level metrics along different chains in a DAG. In particular, we support the following metrics - throughput of each component and throughput, latency and RT along a chain (as defined in \ref{chal:low-level-needs}).

Our approach, \oursys, therefore, requires an input objective function in the form of constraints or weights across these metrics for an application. An example objective for the navigation DAG could be to minimize the weighted sum of response time along different chains, with a higher weight for the local chain to prioritize collision avoidance. As discussed in \ref{chal:low-level-needs}, such requirements will need to be specified by domain experts / application developers, and we discuss the specific requirements we use for different applications in evaluation (\S\ref{chp:eval}). But, we do believe that specifying preferences and constraints on low level is more intuitive and generalizable than directly setting system configuration parameters that could vary with resource usage and availability. In future, we plan to explore whether the mapping from application-level performance goals and the lower-level per-chain metrics can be learnt via offline profiling.

Given an input objective function for an application DAG, \oursys makes CPU scheduling decisions so as to optimize the specified objective and meet the constraints. We allow the constraints to be soft, i.e. if the scheduler cannot meet them, it prints a warning, and aims to meet a looser (scaled up) set of constraints.

We divide the application DAG into \emph{subchains} and make the scheduling decisions at the granularity of each subchain. Each subchain is a series of nodes that run at the same rate in an event-driven manner (with the output from one node triggering the next). Two components A,B can be combined into a single subchain if (a) node B is the only node that consumes data incoming from node A, and there's no value in re-running node B unless there's a new output from A, regardless of B's other inputs, or (b) a particular chain's response time (or latency) constraint is very tight, in which case making a subchain helps by allowing lower delays due to asynchrony between the nodes. Lastly, a node which has drastically unique requirements, such as map callback which 'streams' laser scan inputs, we consider it as an independent subchain.

% TODO: Subchains!!!!?????
% [how to get the mapping bw perf metrics and low level metrics]
For each subchain, \oursys must determine: (i) the number of CPU cores that must be assigned to it, (ii) the degree of per-node parallelism (for multi-threaded nodes), (iii) the rate at which the subchain (source node) is triggered, and (iv) the temporal allocation of CPU across subchains sharing the same core. This is a hard scheduling problem. Even a DAG scheduling involving a small subset of these dimensions has been proven to be NP-hard ~\cite{supplementary-proofs}. We tackle it by adopting an hierarchical approach, where we break our scheduling decisions into two stages -- the first stage determines the mapping between subchains and cores (\S\ref{sec:multicore}), and the second stage makes scheduling decisions at per-core and per-subchain granularity (\S\ref{sec:singlecore}). We begin with outline our approach under the assumption that the computation time at each node and the number of cores is constant, and discuss how we handle dynamicity in \S\ref{sec:dynamicity}. 

% \vspace{-2em}
\subsection{Stage I: Core Allocation}
\label{sec:multicore}
For a DAG with $n$ subchains on a system with $k$ cores, our first stage of optimization outputs a boolean matrix of size $n \times k$, where an element $a_{ij}$ is 1 if subchain $i$ is allowed to execute on core $j$. We use $c_x$ to denote the compute time of node x, and $x \in SC_i$ is the set of all nodes which belong to subchain i. We assume that all cores are homogeneous, i.e. equally powerful, but our approach can easily be extended to handle heterogeneous cores.

\paragraphi{Assumption A1} We make a key assumption for tractability: each subchain either runs alone on a certain number of cores or shares a single core with other subchains (i.e. two or more subchains do not share two or more cores). This helps us in both solving the problem and  simplifying the implementation of the schedule, since each CPU core has an independent run queue to store its tasks, in Linux.

We further make two approximations in this first stage: 

\paragraphi{Approximation Ap1} When multiple subchains share a core, each subchain gets an equal share. This was inspired by the design of Linux' Completely Fair Scheduler, which ensures fairness by distributing the CPU time equally among tasks.

\paragraphi{Approximation Ap2} When a subchain is assigned multiple cores, all of its nodes have the same degree of parallelism (denoted by $q_i$ for subchain i). If the subchain allow parallelism (denoted by $P_i$) \footnote{true if all nodes in the subchain are parallelizable}, we assume that the execution time for all the nodes in the subchain scales perfectly with $q_i$ (i.e. $c'_i = c_i / q_i$).

 We forgo these approximations when making finer-grained scheduling decisions in \S\ref{sec:singlecore}. We develop analytical models to compute per-chain latency, throughput, and response times as a function of $a_{ij}$. Combining with the approximations, we are able to formulate a Mixed Integer Linear Program (MILP) that solves for $a_{ij}$ so as to minimize the specified objective function and meet constraints. We now discuss the formulation in detail.
% Let C denote the number of chains in the DAG. We denote by $l_c$ and $t_c$ the latency and period (i.e. reciprocal of throughput) along a chain, and by $p_s$ the period of subchain s, and by $|c|$ the length of chain c. M denotes a very large number (we use 50,000 in our implementation).

% % \vspace{-1em}
% \setcounter{equation}{0}
% \begin{align}
% \text{min} & \sum_{c=1}^{C} (w_{1c} * l_c + w_{2c} * t_c) + \sum_{s=1}^{n} w_{3s} * p_s &  \\
% \text{s.t.} \sum_{j=1}^k a_{ij} & \geq 1.0 & \forall i \\
%  \sum_{i=1}^n a_{ij} & \geq 1.0 & \forall j \\
%  \sum_{j=1}^k a_{ij} & \geq 1.0 - M*( 1 - x_i) & \forall i \\
%  \sum_{j=1}^k a_{ij} & \leq 1.0 + M*x_i & \forall i \\ 
%  y_{ij} & \leq a_{ij} & \forall i,j \\
%  y_{ij} & \leq x_{i} & \forall i,j \\
%  y_{ij} & \geq x_i + a_{ij} - 1 & \forall i,j \\
%  \sum_{i=1}^n a_{ij} & \leq 1 + M(1 - y_{ij}) & \forall i,j \\
%  \sum_{i=1}^n a_{ij} & \geq 1 - M(1 - y_{ij}) & \forall i,j \\
%  z_{ij} & \leq M(a_{ij}) & \forall i,j \\
%  z_{ij} & \leq p_i & \forall i,j \\
%  p_i - z_{ij} & \leq M(1 - a_{ij}) & \forall i,j \\
%  \sum_{j=1}^{k} z_{ij} & \geq (max_{x \in SC_i} c_x)*b_i & \forall i \\
%  1 - Mx_i & \leq b_i \leq 1 + Mx_i & \forall i \\
%  \sum_{j=1}^{k} z_{ij} & \geq \sum_{x \in SC_i} c_x & \forall i \\
%  w_{ijl} & \leq a_{ij} & \forall i,j,l
% \end{align}

% \begin{align}
% w_{ijl} & \leq a_{lj} & \forall i,j,l \\
%  w_{ijl} & \geq a_{ij} + a_{lj} - 1.0 & \forall i,j,l \\
%  p_i & \geq (\sum_{x \in SC_i} c_x) * (\sum_{l=1}^{n} \sum_{j=1}^{k} w_{ijl}) - Mx_i & \forall i \\
% \text{if not $P_i$ : } b_i & = \sum_{j=1}^{k} a_{ij}  & \forall i \\
%  ex_i & \geq p_i - Mx_i & \forall i \\
%  ex_i & \geq \sum_{x \in SC_i} c_x & \forall i
% \end{align}

% Equation 5.1 represents the objective function, which is a weighted linear sum of the low level metrics. The parameters $w_{1c} \& w_{2c}$ represent the weights for the latency and period of chain c respectively. $w_{3s}$ represents the weight for the period of subchain s. 

% Eqn. 5.2 and 5.3 represent that each subchain (core) should be assigned at least one core (subchain) respectively.

% $x_i$ denotes whether a subchain gets more than one cores, and Eqn 5.4 and 5.5 represent this. Equations 5.6 - 5.8 enforce that $y_{ij} = a_{ij} \&\& x_i$, since $y_{ij}$ represents whether subchain i is on multiple cores ($x_i$) and core j is one of them ($a_{ij}$). Equations 5.9 - 5.10 denote that if $y_{ij} = 1$, then there should be only one subchain on core j. All these eqns together enforce our assumption A1.

We analytically lower bound the period of each subchain based on the $a_{ij}$ parameters. Lets take two cases:

\paragraphi{Case 1} If a subchain gets $\sum_{j=1}^{k} a_{ij}$ cores to execute, then $q_i = \frac{\sum_{j=1}^k a_{ij} }{b_i}$ would be the degree of parallelism i.e.  we allow each node in the subchain to use at most $q$ cores. As per approximation Ap2, we assume each node's compute time scales perfectly with q [which we forgo in \S\ref{sec:singlecore}], and and the period is given by $p_i = max(max_{x \in SC_i} (c_x / q_i), \Sigma_{x \in SC_i} (c_x)/b_i)$. This formula was inspired by our theoretical result of optimal response time for a single chain on multiple cores, explained in more detail in \S\ref{sec:singlecore}. We encode this formula (eqn 5.14, 5.16) in our formulation by making extra variables $z_{ij} = p_{i}a_{ij}$ (Eqns 5.11 - 5.13). Eqn 5.15 signifies that $q_i = b_i = 1$ if the subchain is on a single core, eqn 21 states that $q_i = 1$ and consequently $b_i$ is the number of cores alloted to the subchain, if it is not parallelizable. The MILP solver will make the trade off of $q_i$ while solving for $a_{ij}$; a larger $q_i$ may reduce per-node processing times, but also reduces the degree of pipelining along the subchain. Note that we didn't directly use the $q_i$ parameter in our constraints so as to be able to linearize the formulation.

\paragraphi{Case 2} If a core has $s = \sum_{i=1}^{n} a_{ij}$ subchains assigned, then, due to approximation Ap1, each subchain i gets $1/s$ share of the CPU, and hence will finish one execution in time $(\sum_{x \in SC_i} c_x) * s$. This is represented in eqn 5.20, where in, if subchain i doesn't have $>1$ cores, we lower bound the chain's period by the product of the compute time of the subchain multiplied to the total number of subchains on its core. To help express this constraint in a linear form, we make extra variables of the form $w_{ijl}$, which represent if subchain i and l share core j [represented in Eqns 5.17 - 5.19]. Note that we forgo this approximation in \S\ref{sec:singlecore}, wherein we design a fine grained scheduling policy for each such core.

% The variable $ex_i$ represents the execution time of a subchain i, i.e. how long does it take to finish one full execution \& produce an output. It is at least the total compute time of the subchain (eqn 5.23), and is equal to the subchain's period if it is on a single core (eqn. 5.24) [one could get a tighter bound but we use this approximation].

% Let chain c be denoted by $s_{c0}, s_{c1}..$. Eqn 5.24 and 5.27 describe the chain throughput and latency as a function of other variables. We add constraints corresponding to the following : $LT_x$ ($LT_c$) and $UT_x$ ($UT_c$) represent the lower and upper bounds on the throughput of node x (chain c) respectively. $LL_c$ and $UL_c$ similarly represent the lower and upper bound constraints on the chain c's latency. We can also add constraints/ weights on the chain's response time, which we approximate as $l_c + t_c$. Eqns 5.25, 5.26 and 5.28 represent these constraints.
% \vspace{-0.1em}
% \begin{align}
% t_c & \geq p_i & \forall SC_i \in C_c \\
% LT_c & \leq t_c \leq UT_c & \forall c \\
% LT_x & \leq p_i \leq UT_x & \forall x \in SC_i \\
% l_c & \geq ex_{c0} + \sum_{r=1}^{|c|} ex_{cr} + p_{cr} & \forall c \\
% LL_c & \leq l_c \leq UL_c & \forall c
% \end{align}

\subsection{Stage II: Per Core \& Per Subchain Scheduling}
\label{sec:singlecore}
Given the subchain to core mappings from our first optimization stage, the next stage makes finer-grained scheduling decisions for each subchain and core. There are two distinct cases to consider: 

\paragraphb{Single subchain on one or more cores} We shall now extend the approach mentioned in \S\ref{sec:multicore} (Case 1). Considering a subchain of nodes $\{n_1, n_2, \ldots n_m\}$ with $k$ assigned cores. The scheduler must determine the rate (or the time period $p$) of the source node ($n_1$) and the degree of parallelism for each node, such that the response time is minimized. We allow each node in the subchain to use at most $q$ cores (only a subset may be designed to use all $q$), and set $p = max(max_{j=1}^m (c^q_j), \Sigma_{j=1}^{m} (c^q_j)/\lfloor k/q \rfloor)$, where $c^q_j$ is $n_j$'s computation time with at most $q$ cores \footnote{Note that we are not assuming perfect scaling here, and can use the actual/empirical compute time of each node given q cores}. We have proved that this rate allocation achieves response time (for this particular subchain) within $2 \times$ the optimal, and equal to the optimal for $q = 1$~\cite{supplementary-proofs}. The value of $q$ ranges from $1$ to $k$; a larger $q$ may reduce per-node processing times, but also reduces the degree of pipelining along the subchain. The scheduler iterates over all $k$ choices for this subchain, and selects the value of $q$ that results in lowest response time for this subchain.

\paragraphb{Multiple subchains on a single core} For subchains  $s_1, s_2 ...s_n$ assigned the same core $Q_j$, the scheduler must determine the temporal allocation of CPU time across them. We define a variable $f_i$ for each subchain, which denotes two things: a) the subchain gets $\Sigma_{x \in SC_i} (c_x) * f_i$ CPU time per period, b) the subchain finishes one execution per $1/f_i$ periods. The total period of this schedule then comes out to be $\sum_{i \in C_j} f_i * (\Sigma_{x \in SC_i} (c_x))$. The execution of each (fractional) subchain within a period follows topological ordering. Such a schedule ensures that the CPU core is fully-utilized~\footnote{We can generalize our solution to not use the full CPU if the robot needs to save battery life and the required performance can be achieved with less than a core : add fake node}, while the fraction variables tune the core allocation across subchains. We distinguish between subchains (or nodes) which have constraints on average throughput (e.g. streaming nature such as GML) from others, by allowing f to take arbitrary values for such nodes, but constraining it to be integral - reciprocal (i.e. $1/f_i$ is an integer) for other nodes. This is because, $1/f_i$ being integral allows the scheduler to control the exact throughput of the subchain.

We approximate the per chain metrics as an analytical function of these fraction variables, and formulate a Geometric Programming problem to compute these variables such that the specified objective function is optimized. 
% We now describe our formulation. 
Note that we make a single GP problem to solve for temporal CPU allocation of all the cores. 
% Let SN denote the set of subchains of the streaming nature, and let $Q_j$ denote core j, and $SQ_j$ denote the set of all the subchains sharing core j. 
% \vspace{-0.05em}
% \begin{align}
% \text{min} & \sum_{c=1}^{C} (w_{1c} * l_c + w_{2c} * t_c) + \sum_{s=1}^{n} w_{3s} * p_s &  \\
% \text{s.t.} f_i & \leq 1.0 & \forall x \notin \text{SN} \\
% p^q_j & \geq \sum_{i \in SQ_j} (f_i * \Sigma_{x \in SC_i} (c_x) )  & \forall j 
% \end{align}
% \begin{align}
% p_i & \geq \frac{1}{f_i} * p^q_j & \forall i \in SQ_j \\
% % f_i * () & \geq 1.0 & \forall i \\
% t_c & \geq p_i & \forall SC_i \in C_c \\
% LT_x & \leq p_i \leq UT_x & \forall x \in SC_i \\
% l_c & \geq p_{c0} + \sum_{r=1}^{|c|} 2*p_{cr} & \forall c \\
% LT_c & \leq t_c \leq UT_c & \forall c \\
% LL_c & \leq l_c \leq UL_c & \forall c
% \end{align}
% \vspace{-0.1em}
% $p^q_j$ denotes the period of core j, and its formula is given by Eqn 5.31. Eqn 5.32 represents that each subchain finishes one full execution in $1/f_i$ periods of its core.

% Eqns 5.33 and 5.35 describe the formulae for chains' throughput and latency (similar to \S\ref{sec:multicore}), and Eqns 5.36, 5.37 represent lower and upper bound constraints on these chain level metrics. We similarly can add constraints on node throughput using eqn 5.34. Note that the lower bound constraints are not tight here, i.e. $p_i \geq LT_x$ does not necessarily imply that the the subchain's period (eqn 5.32) will also be more than $LT_x$. This is mostly because geometric programming only supports less than constraints to maintain convexity.

% streaming nodes: fi >= 1, extra pi variable for period if chain ke along : diff empirical period.

% mention pi >= X is not a 'tight' constr.
\vspace{-0.85em}
\section{Handling Dynamicity}
\vspace{-0.25em}
\label{sec:dynamicity}
\paragraphb{Coarse Grained Dynamicity} We handle dynamicity by recording the computation time across all nodes and tracking the number of available cores over time. We re-compute the stage II scheduling decisions (\S\ref{sec:singlecore}) periodically (every 5s in our implementation) using the 95\%ile computation time for each node measured over the previous 50 values in our implementation (We support multimodal compute times by taking the weighted sum of 95\%ile compute times across the different modes). We re-invoke the stage I optimization (\S\ref{sec:multicore}) less frequently (once every 20s in our implementation). We chose these periods so as to keep the overhead of re-solving low.

\paragraphb{Fine Grained Dynamicity} We are exploring using priorities or precedence as a way to handle fine grained variations, e.g. sudden spikes in compute times. For instance, we can specify if a node B wants to wait for a new output from another node A \footnote{This is almost a middleground between B being independently frequency driven and being synchronous w.r.t. A}. This will allow node B to take up some of the cpu time assigned to node A if needed. We can add extra constraints in our optimization problems to reflect this as well.

We add extra constraint on the each subchain $c_i * f_i \geq 1$ to limit the overhead, which limits the hyper period of the core to be atleast the number of subchains executing on the core. We can extend the fractional policy by allowing only a subset of nodes/subchains to run each hyper period, so as to support faster periods with less overhead.

% coarse grained -> re-solve if 5s [decided to keep overhead low] or if smt changes suddenly [not more than 1hz].

% fine grained -> priority based.

==> old/introduction-old.tex <==
Sense - react systems such as robotics and AR/VR  are becoming ever more pervasive. While  a variety of robots now assist us with various mundane, high precision, or dangerous tasks~\cite{roomba, kiwi, amazonrobotics, surgrobot1, surgrobot2, surgrobot3, drone-fire, waymo, tesla}, XR has affected the way we teach, practice medicine ~\cite{surgeon-xr, vr-neuro}, etc, and is envisioned to be the next interface for compute ~\cite{HuzaifaDesai2020, nvidia-xr}. 
Both robots and XR systems typically feature a sense-perceive-plan-react pipeline (Figure~\ref{fig:basicpipeline}) which ranges from a single linear chain of components in the simplest applications to a multi-chain directed acyclic graph (DAG) in more complex ones. Most such systems run on devices with limited compute, e.g. a mini PC~\cite{locobot, terrasentia} or Raspberry Pi~\cite{turtlebot3-pi, turtlebot3} or 
% Run on edge systems : limited compute and memory resources. \todo{!!}
In this work, we motivate the need for automated and dynamic resource management in such compute platforms, identify the key challenges, and develop a preliminary scheduling framework to dynamically manage on-device CPU resources for sense - react systems at runtime.

Resource management for robotics and AR/VR requires co-optimizing multiple dimensions -- how much resources must be allocated to each component, how often each component gets triggered, and the order in which they run. This results in a difficult scheduling problem, where the appropriate choice depends on the amount of available resources, the resource usage of each component, and the performance requirements of the application. The resource manager must also take into account dynamic variations in resource usage (e.g. due to accumulation of more information about the environment, or a change in scene) and in resource availability (e.g. due to battery constraints). The fact that the impact of scheduling decisions on the performance
% requirements 
of a sense react system 
is deeply tied to semantics of the specific application, further add to the difficulty of resource management.

Despite the rich literature in system scheduling, past work fall short of addressing these requirements and challenges in sense - react systems. They either optimize a subset of the dimensions listed above (e.g. just the triggering frequency ~\cite{davare2007period}, or the execution ordering ~\cite{yang-priorities, waters-priority, rosch-rt-e2e-lat}), or consider local (per-component) adaptations that do not take system-wide requirements into account \cite{aurora-load-control, borealis, seda, zeromq, rabbitmq, seda-followup, heron}, or rely on static configurations learnt offline that cannot adapt to dynamic variations  \cite{opentuner, automagic, bo4co, videostorm, auto-clustersz-hadoop}. To the best of our knowledge, none of the related works discuss the correlation between scheduling decisions and applications' performance.

Thus resource management in sense - react systems remains a challenge in which developers are provided little help. While frameworks that assist in development of applications exist (e.g. ROS~\cite{ros}, ILLIXR ~\cite{HuzaifaDesai2020}, OpenXR ~\cite{openxr}, they leave resource management decisions entirely up to the application developers in the form of manually configurable parameters. Application developers often react to poor performance with desperate attempts at fine-tuning the scheduling decisions for different components, scaling up the resources, and other such ad hoc strategies. The engineering effort involved in hand-tuning system performance steals from the time that could have been better spent on developing more useful higher-level applications, and also increases the barrier of entry into the field of robotics and AR/VR.

We therefore highlight the key scheduling challenges and requirements, and design \oursys(\S\ref{sec:design}), an automated resource manager to dynamically manage the compute resources for a sense react application. 
% without requiring low-level configurations from the application developers. 
\oursys uses a hierarchical approach to solve the scheduling problem, and has support for handling various kinds of application requirements. It can be plugged into existing robotics and AR/VR frameworks (e.g. ROS, ILLXIR respectively), and provided as an optional service to the applications using the framework. Through our preliminary case studies (\S\ref{sec:eval}), involving 3 applications in both domains (object tracking robot, exploration robot and Virtual Reality), 
% implemented in ROS and evaluated using standard robotics simulators~\cite{gazebo, Stage}
we show how \oursys can achieve better application performance than the default (hand-tuned) configurations, and demonstrate the significance of meeting the scheduling requirements, specifically handling dynamicity and heterogeneity in the DAG.
% dynamically adapting to resource usage variations over time. 
To the best of our knowledge, this is the first work to evaluate the impact of system scheduling on how well a sense - react system fulfills its tasks.

Our work thus motivates the need for automated resource management at runtime in order to improve a system's performance and ease application development. While, as a first step, we focus on managing CPU resources on the edge device for robots / XR, our work opens up several interesting directions for future research (\S\ref{sec:concl}), which include generalizing to systems with heterogeneous compute resources (e.g. CPU, GPU), simultaneously managing memory and network constraints, and to other sense-react applications.
